Perils of Zero-Interaction Security in the Internet of Things

The Internet of Things (IoT) demands authentication systems which can provide both security and usability. Recent research utilizes the rich sensing capabilities of smart devices to build security schemes operating without human interaction, such as zero-interaction pairing (ZIP) and zero-interaction authentication (ZIA). Prior work proposed a number of ZIP and ZIA schemes and reported promising results. However, those schemes were often evaluated under conditions which do not reflect realistic IoT scenarios. In addition, drawing any comparison among the existing schemes is impossible due to the lack of a common public dataset and unavailability of scheme implementations. In this paper, we address these challenges by conducting the first large-scale comparative study of ZIP and ZIA schemes, carried out under realistic conditions. We collect and release the most comprehensive dataset in the domain to date, containing over 4250 hours of audio recordings and 1 billion sensor readings from three different scenarios, and evaluate five state-of-the-art schemes based on these data. Our study reveals that the effectiveness of the existing proposals is highly dependent on the scenario they are used in. In particular, we show that these schemes are subject to error rates between 0.6% and 52.8%.

==> section/results-removed.tex <==
\subsection{Insights from the raw data}
\label{sec:res:rawinsight}
Before investigating the performance of the different \gls{zia} systems, we explore the collected raw data from the Car and Office experiment.
This can serve to give an intuition for which types of features we would expect to work well in these scenarios, and thus inform future context feature design.


\subsubsection{Office}
\label{sec:res:rawinsight:office}
\change{This part will probably be moved to the appendix}We observed the \textit{barometric pressure} to be very close for all sensors, regardless of the office.
This is to be expected, since all offices were on the same floor of the building.
The \textit{humidity} inside single offices follows the same trend, but the absolute values are often offset from one another.
%TODO Need a better word than "trend" here (and in all other places)
We also observe that the trends of the humidity readings differ between offices, likely depending on doors and windows being opened and closed at different times.

The \textit{luminosity} readings within a single office share the same trends for most of the sensors, aside from those in dark places like the cupboard.
Devices that are closer to natural sunlight show larger peaks in their luminosity measurements, which are shared across sensors on the same side of the building (i.e., offices 1 and 2).
For offices on opposite sides of the building, trends are still often quite similar, but show different amplitudes depending on the position of the sun relative to the office windows.
Office lamps provide an artificial baseline luminosity that is similar between offices.
At night, the luminosity is zero for all devices.

The \textit{temperature} readings also show similar trajectories within an office, matching the increases and decreases of colocated sensors, but often offset from one another, sometimes by up to 6 degrees celsius, depending on their position.
The temperature varies between the different offices, and changes are mostly related to factors within the office (e.g., opening or closing windows).
Thus, the measurements show a much lower variation at night.

The \textit{audio} recordings show the expected frequency ranges for a busy office, with the addition of a background noise level in the low frequencies (below 500 Hz)\change{This is probably wrong}, which is likely due to electrical interferences between devices during the recording.

\textit{WiFi} and \textit{BLE} measurements show strong variations even on shorter time intervals, as the 2.4 GHz spectrum used by WiFi and BLE is being taxed by the many BLE connections used by the sensors to transmit their data to the Raspberry Pi's.
This leads to sporadic interference with the beaconing done by the WiFi access points.
We can still observe that, on average, sensors in some positions (on lamps and walls, near windows) will see more WiFi beacons than those in more hidden positions (cupboard, screen), with the counts varying by up to 50\% in some cases.

The differences are less pronounced for BLE measurements, where the counts are much more similar over time.
We also observe that the number of observed BLE devices was strongly dependent on the time of day, with almost no devices visible during the night when the offices were empty.

%\begin{itemize}
%	\item Within-Office
%	\begin{itemize}
%		\item \textbf{Barometric pressure} follow the same trend, with small offsets between the sensors (measurement accuracy ftw).
%		\item \textbf{Humidity} follows similar trends, but at different base levels. Individual sensors may also exhibit spikes and drops that are not always closely followed by other sensors in the same office.
%		\item \textbf{Luminosity} is a bit of a special case. Most of the devices follow roughly the same trends. However, the devices that are exposed to direct sunlight (i.e., windows) have much larger spikes than the others, and also show a much larger variance in their values. Naturally, the devices in the cupboards show very little impact from the light and stay very low.
%		\item \textbf{Temperature} once again follows similar trends, but at very different base levels. Temperature can differ by up to 6 degrees celsius within the same office. However, it actually translates surprisingly well to devices hidden in cupboards etc.
%	\end{itemize}
%	\item Between-Office
%	\begin{itemize}
%		\item \textbf{Barometric pressure} exhibits the same trends, often offset from one another.
%		\item \textbf{Humidity} often shares long-term coarse trends, but does not match all the small jiggles that appear over the day
%		\item \textbf{Luminosity} is in many cases similar in magnitude for devices on the same side of the building. The other side of the building tends to share some of the changes, but not all. room lighting also plays a role (if it is switched off at different times), but is otherwise constant and in many cases at similar levels.
%		\item \textbf{Temperature} is more dependent on factors within the office than global factors. Especially opening the window tends to have a big influence, as you may expect. The side of the building plays less of a role than expected.
%	\end{itemize}
%\end{itemize}
%Audio: Expected frequency ranges for a busy office. During the night, a (microphone-induced) noise is observed, which stays below 500 Hz most of the time.


\subsubsection{Car}
\label{sec:res:rawinsight:car}
\change{This part will be probably moved to the appendix}As before, the \textit{barometric pressure} generally follows the same trends for all sensors, regardless of the car, with a slight offset between the sensors.
However, this changes as soon as the two cars separate - with a growing distance between the cars, the measurements also become offset from another, owing to the different altitudes on the hilly roads.
Thus, we can see that, as expected, the barometric pressure difference depends on the geographic proximity of the cars.

The \textit{humidity} shows a high correlation within the individual cars, although the values are offset from one another by up to 10 percentage points.
The humidity initially drops before stabilizing at an approximate baseline level of between 25 and 15 \%, but still shows some variation.
The curve is noticeably smoother while the car is turned off and not occupied.

\change{Shorten this part}The \textit{luminosity} depends on the position of the sensors within the car.
The devices on the dashboard, which are exposed to direct sunlight, match their luminosity readings very closely while the cars are travelling together, and only deviate after the cars have separated.
As expected, the sensors in the glove compartment show almost no measured luminosity.
Those located near the handbrake show significant readings in one car, while showing almost no luminosity in the other. This can be explained by the positioning - in one case, the sensor faced upwards, while in the other, it faced backwards in a 45-degree angle and thus away from the light coming in through the windshield.

The sensors on the handles in the back of the car showed similar trends between the two cars, but with different amplitudes.
Those in the trunk differ greatly between the cars, as in one of the cars the light was blocked by the hatch.
Aside from trunk and glove compartment, the luminosity readings within a car were following similar trends with different amplitudes and some small deviations.

The starting values of the \textit{temperature} are surprisingly far apart, with differences of up to 4 degrees within the same car.
While driving, the overall trends within the same car are similar, but not consistently so.
Notably, the sensor in the glove compartment appears to be almost completely decoupled from the temperature of the other sensors, owing to the constrained space and lack of air circulation.
At the beginnisectionng, the temperature increases on all sensors, likely due to a combination of the AC system of the car and the heat dissipation of the sensor devices.
Once a steady-state has been reached, the variation is usually quite low, and larger changes can be explained by outside actions (opening the window or doors, changing the temperature on the AC).
This also means that the similarity between different cars is quite low.

The \textit{audio} spectrum shows a pervasive hum while the engine is running, with other frequencies mixed in based on the speed of the car and the surface it is travelling over. 
For most sensors, this dominates the spectrum, with speech, music and other factors being more or less drowned out, depending on the position inside the car.

The \textit{WiFi} and \textit{BLE} captures within a single car show similar large-scale behaviour, although there are still observable deviations between the sensors (i.e., specific broadcasts are seen by some, but not all devices).
The similarity between devices in different cars is also quite high, as long as the cars are driving close together.
As expected, the differences become much larger as soon as the cars separate.


%\begin{itemize}
%	\item Within-Car
%	\begin{itemize}
%		\item \textbf{Barometric pressure} follows the same trend, but with a difference of up to 1.7 (unit?) between the sensors. Bigger differences in car 1, biggest between S1/2 and S4.
%		\item \textbf{Humidity} is quite variable, following mostly similar large-scale trends, but not consistent (see S1 vs S3, falling vs. rising on the rest stop, i.e. converging towards a specific value?). Shows an initial large drop before stabilizing on different levels. Trends differ between cars.
%		\item \textbf{Luminosity} shows that the largest spikes are observed on sensor 1 and 7 (on the dashboard). The others show marginal changes, although car 2 shows larger changes than car 1
%		\item \textbf{Temperature} starts at surprisingly different levels (up to 4 degrees different). Similar large-scale trends, but different steady-state temperatures. Also obviously depends on position.
%	\end{itemize}
%	\item Between-Car
%	\begin{itemize}
%		\item \textbf{Barometric Pressure} is quite similar for pairs of sensors in the same position (sometimes time shift due to bad sync observed).
%		\item \textbf{Humidity}, as expected, shows differences in this evaluation as well (not surprising, if it can't even agree within the same car)
%		\item \textbf{Luminosity} on the dashboard is very close together, in others it varies. implication: Direct exposure to sunlight tends to sync them up fairly well, indirect light is harder to sync.
%		\item \textbf{Temperature} shows similar trends in terms of starting up and cooling down. Steady-state does not show universally similar trends.
%	\end{itemize}
%\end{itemize}


\subsubsection{Implications for context feature design}
\label{sec:res:rawinsight:implications}
\change{Rewrite, restructure after moving previous subsects to appendix}
Given these observations, we can see that \textit{barometric pressure} appears to be suitable for coarse-grained location checks (determining separations on the scale of kilometers), but unsuitable for fine-grained separation of contexts (e.g., different rooms of the same building).
Additionally, it shows a low variance and slow changes over time, making it potentially easier to spoof.
Nevertheless, a low absolute difference between measured values may serve as a weak indicator of co-location, which could be strengthened through multiple consecutive observations over a longer timeframe, if the application domain allows it.

\textit{Humidity} shows a good potential for separating even very proximate contexts, like two neighboring offices, as long as the used feature can also capture smaller variations over time.
The large offsets between measured values even in the same office and car indicates that capturing trends over a longer amount of time would be a more promising approach than taking absolute differences of individual values.
It should be noted that this only applied to areas with a lot of variation in humidity, like occupied offices, as we have seen that empty offices have a much lower variation over time and tend to converge towards a steady-state value, which may be easier to spoof.

The \textit{luminosity} shows large variations depending on position and orientation of the sensor.
This makes using absolute differences between values a challenging proposition.
Additionally, natural light sources like the sun do not isolate different offices, while artificial light sources show a low variability and thus make adversarial guessing easier.
If luminosity is used at all, it should be used in a scheme that compares trends over long timeframes, and in settings that ensure that devices have similar visibility of ambient light.
It goes without saying that features based on natural ambient light will fail at night.

The recommendations for systems based on \textit{temperature} follow those for humidity: The context needs to provide enough variation over time (in many cases provided by human activity), and is unsuitable for areas with strict climate control that keeps the area at a specific temperature.
Once again, changes over time may be a better indicator than absolute differences at specific times.
However, the slow rate of change may make gathering enough entropy within a reasonable timeframe a challenging proposition.

Given that many modern environments are built with sound isolation in mind, features based on \textit{audio} are promising.
Their problems lie in other areas, like user acceptance of temporary or even persistent sound monitoring, which may be unacceptable or even illegal in certain contexts (e.g. banks, hospitals, ...).
The features should also be able to deal with persistent background noises - while the engine noise in our example may help in separating the two cars, the risk is that two cars of the same make and model may have very similar engine noises, thus risking an incorrect pairing between them.

Features based on \textit{WiFi} and \textit{BLE} are promising for coarse-grained separations, since WiFi is already being used for geolocation.
The possibility of a more fine-grained separation of neighboring offices may be more challenging, depending on the density of devices, the quality of the receivers, and the saturation of the wireless spectrum - our experiments have shown that a saturated spectrum can lead to unreliable delivery of WiFi access point beacons, leading to discrepancies in observed networks over time.
Additionally, some areas (like rural areas or highways between cities) may have no observable wireless access points.

BLE encouters the additional problem that the observed devices are mobile.
This means that certain environments may have BLE devices to facilitate context comparisons at certain times of the day, but not at night, leading to the scheme breaking down in these situations.
This is less likely for WiFi, where almost all access points are installed in fixed locations and running 24/7.

Having discussed the basic properties of the observed data, we will now investigate how the five reproduced schemes performed in our two scenarios.




\subsection{Performance insights}
\label{sec:perfaudio}
\change{Remove completely}
%TODO Proposal: If there is no difference in performance between colo and noncolo devices, just state it and don't spend too much time on it.
To compare the performance of different audio features that we re-produced \citep{Schurmann:2013, Truong:2014, Miettinen:2014, Karapanos:2015} we ran a set of benchmarking tests for both car and office scenarios. 
We wanted to check if there was any difference in audio feature performance among devices in the same application context and in different contexts, as well as, to find out if random and aligned audio samples had any effect on audio feature performance. 
For that we generated two classes of audio samples: random and aligned for car and office scenarios. 
Concretely, for the random samples we took random audio chunks for each time interval that we considered (i.e. 5 sec -- 2 min), from the each sensor's audio recordings used in our evaluation. 
The aligned audio chunks were sampled randomly on the basis of different time intervals, but within each time interval each audio chunk was obtained from the same position in each sensor's audio recording. 
Note that for the car scenario we used full audio recordings for each sensor, e.g. 3 hours, for the office experiment we generated samples from the first 24-hours of audio recordings. 
Thus, for the car scenario for each class (random or aligned) we obtained 6*12=72 audio chunks, i.e. 6 chunks per sensor for each time interval (5sec, 10sec, 15sec, 30sec, 1min, 2min). 
As stated above, we considered both colocated (30 per time interval) and non-colocated (36  per time interval) audio pairs, which resulted in 66 unique benchmarking runs per time interval, and, overall 6*(30+36) = 396 runs for each class (random and aligned) in the car scenario. 
For the office scenario we had 6*24=144 audio chunks, i.e. 6 chunks per sensor for each time interval, which resulted in  84 and 192 audio pairs for colocated and non-colocated audio pairs, i.e. 276 unique audio pairs per time interval, and, overall 6*(84+192) = 1656 runs for each class (random and aligned) in the office scenario.
The results are...

Table \ref{tab:bm-setting-car} for the car benchmarking setting and Table \ref{tab:bm-setting-office} for the office benchmarking setting.

\begin{table}[!htb]
	\caption{Benchmarking setting for the car scenario}
	\label{tab:bm-setting-car}
	\begin{tabular}{cc|ccc}
		\toprule
		\multicolumn{2}{c|}{Audio samples} &
		\multicolumn{3}{c}{Audio sample pairs} \\
		{Type} & {Number} & {colocated\textsuperscript{*}} & {Non-colocated\textsuperscript{*}} & {All\textsuperscript{**}} \\
		\midrule
		Aligned & 72 & 30 & 36 & 396 \\
		Random & 72 & 30 & 36 & 396 \\
		\bottomrule
	\end{tabular}
	\center{*\textcolor{white}{-}= per time interval; **\textcolor{white}{-}= for all time intervals}
\end{table}

\begin{table}[!htb]
	\caption{Benchmarking setting for the office scenario}
	\label{tab:bm-setting-office}
	\begin{tabular}{cc|ccc}
		\toprule
		\multicolumn{2}{c|}{Audio samples} &
		\multicolumn{3}{c}{Audio sample pairs} \\
		{Type} & {Number} & {colocated\textsuperscript{*}} & {Non-colocated\textsuperscript{*}} & {All\textsuperscript{**}} \\
		\midrule
		Aligned & 144 & 84 & 192 & 1656 \\
		Random & 144 & 84 & 192 & 1656 \\
		\bottomrule
	\end{tabular}
	\center{*\textcolor{white}{-}= per time interval; **\textcolor{white}{-}= for all time intervals}
\end{table}

